RD50-MPW3: A fully monolithic digital CMOS sensor for future tracking detectors

The CERN-RD50 CMOS working group develops the RD50-MPWseries of monolithic high-voltage CMOS pixel sensors for potential use in future high luminosity experiments such as the HL-LHC and FCC-hh. In this contribution, the design of the latest prototype in this series, RD50-MPW3, is presented. An overview of its pixel matrix and digital readout periphery is given, with discussion of the new structures implemented in the chip and the problems they aim to solve. The main analog and digital features of the sensor are already tested and initial laboratory characterisation of the chip is presented.

==> overview.tex <==
\section{Key Facts of RD50-MPW3}
Rd50-MPW3 has been designed using the LF15A process from LFoundry. Apart from the standard resistivity, the chip has been manufactured on high resistivity wafers using a 1.9\,kOhm\dot cm and a 1.9\,kOhm\dot cm substrate. As seen in figure \ref{fig:picCHIP}, the main area of the chip consists of an 64 by 64 pixel matrix which a pixel size of 62\,\textmu m by 62\,\textmu m, which gives an active area of around 4\,mm by 4\,mm. A digital periphery for readout and control is located on the bottom of the chip. The overall chip size is 5.1\,mm by 6.6\,mm.

\begin{figure}[!ht]
    %\captionsetup{skip=1pt}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/picture_chip.png}
    \caption{r}
    \label{fig:picCHIP}
\end{figure}
